React to This! How Humans Challenge Interactive Agents using Nonverbal Behaviors

How do people use their faces and bodies to test the interactive abilities of a robot? Making lively, believable agents is often seen as a goal for robots and virtual agents but believability can easily break down. In this Wizard-of-Oz (WoZ) study, we observed 1169 nonverbal interactions between 20 participants and 6 types of agents. We collected the nonverbal behaviors participants used to challenge the characters physically, emotionally, and socially. The participants interacted freely with humanoid and non-humanoid forms: a robot, a human, a penguin, a pufferfish, a banana, and a toilet. We present a human behavior codebook of 188 unique nonverbal behaviors used by humans to test the virtual characters. The insights and design strategies drawn from video observations aim to help build more interaction-aware and believable robots, especially when humans push them to their limits.

==> Sections/discussion.tex <==
From the recorded non-verbal interaction video and the interview data, several behavioral patterns emerged. First, we summarized the interesting findings for each of the social, emotional, and physical behaviors. Then, we discuss the association between the three categories of behaviors and morphology. In the end, we will uncover the other virtual character design insights.


%Exaggeration is one of the widely known animation principle listed in The Illusion of Life: Disney Animation \cite{thomas1995illusion}, where it is supposed to be followed to make the story
\subsection{Social, Emotional and Physical Behaviors}
\label{subsec: discussion}
\subsubsection{Social Behaviors}
In total, we counted 39 social behavior categories. From the collected 20 participants' data, we observed waves for greeting, thumbs up as a ``good job" compliment carried out by multiple participants to express similar meanings. In addition to these well-recognized behaviors, there were also culture-specific behaviors such as namaste, a greeting gesture performed by pressing hands together, and fingers pointing upwards in the Indian subcontinent. This reminds us of the importance of investigating culture-specific emblematic behaviors in HCI area.

We also found that different behaviors might share similar social meanings. For instances, punching, kicking, and fire handguns all can be used to express one's aggression toward another. The interpretable themes that surfaced from the participants' behaviors provided us with a dictionary to refer to when looking into the emblematic gestures/behaviors (see Appendix).


\subsubsection{Emotional Behaviors}
Firstly, exaggerated actions were seen frequently in emotional behaviors. For example, participants tried to express sadness by finger-drawing a downward curling line in front of their face, moving index fingers from the eye's corner to the chin to depict tear dropping, and rubbing fists around their cheeks to pretend crying hard. The occurrence of such pantomime actions might indicate a low expectation of intelligent virtual characters' capability in emotion recognition. P120 mentioned that the penguin character reminded her of an infant who cannot do much to the external stimuli. This phenomenon might also be explained by compensation for the removal of other communicative modalities (e.g. voice, verbal). As we pay more attention to recognizing precise and realistic emotional expressions in the affective computing area, we should also look into these over-emphasized expressions as they might occur in certain interactive circumstances.

Secondly, we found that one emotion category could comprise multiple unique behaviors. While not surprising based on literature in psychology \cite{barrett2019emotional}, these actions could serve as alternate targets for recognition systems, i.e. instead of attempting to recognize ``sadness", which is an overarching concept comprised of heterogeneous actions, computer vision researchers could aim to recognize ``rubbing eyes, pretending to cry", ``lowered lip corners" and so on.


% \subsubsection{Physical Behaviors}
% We grouped physical behaviors into subcategories as one of the following: posture (lower body, full body, hand, head/face, arm), proxemics, physical contact, and role play. It is possible that the physical behaviors reflected participants' various testing intentions during the interaction:

% \begin{itemize}

%     \item \textbf{Actuation testing.} Participants initiated some interactive behaviors to see if the character was able to follow and replicate. Arms and hands movements were also shown in the interaction session with the character banana, even though it did not have any hands. As shown in Table \ref{tab: physical}, other behaviors included natural movements humans do in real life such as scratching with hand, squatting, and walking in space.

%     \item \textbf{Sensor testing.} In some interactions, characters were not expected to copy the participant's exact movement. For example, P113 put on their hood in front of the robot character. Participants appeared to be testing the sensing abilities of the character and if the characters were aware of their presence and actions, and were curious about the characters' reactions.

%    \item \textbf{Physics testing.} Finally, participant also interacted with the characters where clear physical feedback was anticipated. Actions involving physical contact contributed to these types of behaviors testing physics-based responses, such as lifting, pushing and poking.
   
%    \item \textbf{Role-Playing.} Character specific interactions comprised the bulk of behaviors falling into our ``role-playing" category. These included, for example, swimming and puffing out cheeks for the fish, or waddling for the penguin. It is possible that an element of imaginative or pretend play explained some of these behaviors, projecting the participant into the character's world and movements.

% \end{itemize}


 
%\begin{figure*}[t]
    % \centering
%    \includegraphics[width = 0.9\textwidth]{Figures/sequential.png}
%   \caption{Stimuli consisting of sequential actions}
%    \label{fig:sequential}
    % \Description{Three drawn illustrations for stimuli consisting of sequential actions.}
%\end{figure*}

\begin{figure}[t]
    % \centering
    \includegraphics[width = 0.45\textwidth]{Figures/sequential & multimodal.png}
    \caption{Stimuli consisting of sequential actions (top) and stimuli consisting of combined actions (bottom).}
    \label{fig: sequential_multimodal}
%     \Description{Two drawing illustration pairs for stimuli consisting of combined actions. For each pair, the shared action and meaning of each stimulus is written.
% }
\end{figure}
 % What insights can be gained by analyzing the patterns of non-verbal interactions and interview data
\subsection{Behaviors and Morphology}

Character-specific morphological characteristics appeared to affect the likelihood of character-specific behavior occurrence (Fig. \ref{fig: character-specific}). For example, ``flushing the toilet" and ``pulling the toilet paper" behaviors were only  observed during interaction with the toilet, and not any other character. Similarly, participants only touched and twirled their hair when interacting with the human among all six characters. From our study, one design guideline may be to expect interactions that are relevant not just to general socio-emotional communication, but also to the characters' morphology. In other words, the appearance of a character may afford certain physical interactions. \\

 % For virtual characters used for specific purposes (restaurant serving, tourism, etc.), limited non-verbal interactive capabilities may be acceptable to keep the task more targeted and straightforward. Nonetheless, during free interactions, virtual characters should be able to understand and respond to all possible interactive behaviors that humans might challenge them with.


 As reported in Sec. \ref{subsec:results_morphology}, the behavior frequency counts were not independent of the character conditions. Reflecting on the significant result in $\chi ^2$ test of independence and the large adjusted residuals, we saw a high proportion of \emph{social behaviors} in the penguin and the human conditions. This might be attributed to the fact that these are both characters representing live animals. P111 kindly asked the human character's age during the interaction, and they explained the motivation behind this behavior as ``Like the human,(I) probably would just do something they would understand. I wouldn't ask like the penguin, or the animal, or the banana, or the toilet like how old they were". 
 %We also observed a trend that participants tend to use more social behaviors with characters that are highly animated. 
 A surprising result was that fish, while also an animal, saw the fewest number of social behavior counts. Possible explanations may be related to the perceived intelligence of the species (e.g. fish vs. birds vs. primates).
 %, or the scarf accessory available on the penguin that acted as a non-verbal communication topic. 
% We also notice a high proportion of \emph{physical behaviors} in the fish and toilet conditions. This might be explained by the physical responsiveness in the fish condition (i.e. quick movements) and the varied aspects of the toilet for physical interaction (i.e. toilet flush handle, lid). % Compared to banana, toilet and robot which are perceived as inanimated objects in the real life, human, fish and penguin are highly animated beings. As expected, the later three were ranked in the top 3 positions in terms of animacy scale, or in other words, how lifelike they appear.

  Overall,  general features (e.g. whether the character represents a living creature or object, with/without arms) and specific features (e.g. certain accessory attached to the character) need to be taken into account when trying to exhaust the character's interaction affordance. This design strategy will prevent the human interactor from being disappointed by the mismatch between their expectation of the characters and reality. 
 
 %However, we did not include the character-specific interactive behaviors in our codebook because of their lack of generalizability into the virtual characters in various forms in the wild.

% \subsection{Perceived Interaction Quality and Morphology} Before answering this interview question, participants were asked to rank the characters twice, first based on the interaction quality, and then based on the cuteness level. Thus the participants were primed that interaction quality and perceived cuteness level should be evaluated separately. However, 4 participants still mentioned during the interview that cuteness is one of the attributes they valued a lot when assessing the interaction quality. We also see that in Fig.~\ref{fig: ranking}, the penguin and the fish were ranked relatively high in both cuteness and interaction quality for the majority of the participants.

 
% \subsection{Animacy and Morphology} 
%  Shown in Fig. \ref{fig: animacy_boxplot}, we observed that the statistically significant difference exists only in three pairs: between the robot and the animated characters (the fish, the penguin and the human). It was worth mentioning that two of the Godspeed Animacy scale questions ask participants to rate the evaluated agent on the spectrum of "mechanical-organic" and "artificial-lifelike". This suggests that the Godspeed Animacy scale might not be a proper proxy for interaction awareness in our study, as the robot's morphological characteristics could determine the animacy level regardless how responsive and interactive the robot character was. This finding also reminds us there is a call for a more applicable interaction awareness measuring tool for interactive agents in the future.
% -------------------------------------------------------------------------------

\subsection{Other Observations for Virtual Character Design}
While the goal of this study is to focus on human behaviors within interactions, we describe here some notable feedback from participants regarding the character reactions to their behaviors.

\subsubsection{Mirroring}
% As human beings, when seeing other people, we are able to understand others' actions and emotions by inferring self-performed actions and self-experienced emotions based on our observation of others~\cite{oberman2007simulating}. 
In this study, we saw that participants involuntarily and unconsciously mimicked the characters’ behaviors or derived the next interactive behaviors from the characters’ behaviors.  Fifteen participants mirrored the characters' actions in this study. It is hard to differentiate if those mirrorings are conscious or nonconscious behaviors, so we selected two that were reported by the participants during the interview as examples to discuss. 
P103 reported that after he knocked himself on the head, the banana character appeared to fall asleep (pretending to pass out after being hit), so he tried to do the sleep action in order to examine if the banana actually understood this action and was able to replicate it. During the video annotation process, we saw sometimes participants ran out of interaction ideas, and paused or even stopped interacting with the characters. Consciously mimicking the character's response is one of the methods they used to create more interactive behaviors. 

In 1999, Chartrand and Bargh found that people nonconsciously mimic others' facial expressions and behavioral mannerisms during interaction (the chameleon effect) \cite{chartrand1999chameleon}. This pattern was also found in our study. P101 claimed that because he saw that the human character had hair, he actively chose to test if the character was able to groom her hair as he could. However, from the recorded video, we clearly saw that the character touched her hair, then the participant immediately performed the same action. It appears likely that the participant nonconsciously picked up this spontaneous behavior from our teleoperator behind the screen. This suggests that each action performed by the agent should be listed as an action that the agent also needs to recognize. 

 \subsubsection{Behaviors Consisting of Sequential Actions and Combined Actions}
 We observed that for interactions containing complex meanings, one single gesture/action is not sufficient enough for people to express themselves without speech. As an illustration, the "heart" gesture was used to convey a few different meanings as follows: a) test if the character is able to replicate; b) show their affection; c) compliment. We saw that P119 touching her own hair first, and posing a
heart gesture later to form a sequence of actions to complete the compliment behavior. Thus, being able to segment action sequences and understand them correctly is crucial for the virtual character to respond appropriately. 
 % In Fig. \ref{fig:sequential}, several examples are given.
 
 We also saw participants creating different behaviors by using various combinations of face and body movements. For instance, 
 "shrug" action was seen as a signal of "I don't know/understand" when it was in the company of raised eyebrows, and was perceived as a sign of "tada!" when the participants held the shrug for a long time and wore a surprised and happy face. Sequential and combined actions (see Fig. \ref{fig: sequential_multimodal} for examples) make the segmenting and recognizing behavior achallenging problem. Multimodal action segmentation and behavior interpretation is an important direction for future work toward fully autonomous interactive virtual characters.

% \subsubsection{Expectation} In this study, several participants complained about the lack of expected reactions to certain behaviors. For example, the toilet character did not have a flushing animation and it was hard for the teleoperator to show a proper response to this action. Thus, to respond, the teleoperator always leaned to the right (the flushing handle was on the right), blinked the right eyes, and made a sad face if the participant kept doing the flushing actions for a longer time. Even though these responses were appropriate considering the incapability of flushing, participants still showed their disappointment with the character. Four participants reported that whether the character's responses meet their expectations is a determinant of the interaction quality. \textit{"(P111) Sometimes I did something, and it didn't react in the way that I assumed"}. 

% \subsubsection{Preference for Reaction over Mirroring}
%  We observed that physical tests (e.g. raising arm) generally consisted of a participant trying to see if the character could copy them. However, for social and emotional behaviors, participants were not satisfied when the characters responded to the behaviors in the form of simple mirroring. The teleoperator was instructed to react in a natural way whenever it is possible (a clear meaning was perceived). For example, when the participants peeled or ate the banana, the teleoperator pretended to be angry, turned the body away, and avoided eye contact with the participants. But for behaviors that do not have clearly interpretable meanings, such as folding arms, the teleoperator mirrored the participants' actions. During the post-study interview, a few participants explicitly stated their preference for a natural reaction instead of a straightforward mirroring as the reactions make the characters more lifelike. Thus, when designing a virtual character's default or idling behaviors, reducing the frequency of imitating the human interactors' behaviors and trying to add more reactive behaviors to common interaction behaviors might increase the characters' likeability and perceived overall interaction quality.


% -------------------------------------------------------------------------------




% \subsection{Perceived Control of the Virtual Characters}
% To prevent priming from affecting participants' ratings of the characters, we deceived the participants about the type of control the characters had. Before the interviewer posed the question "Do you think any of the six characters can be teleoperated/controlled by a human?", only two participants suspected that there might be a person puppeteering the characters behind the curtain. P103 reported that as he interacted with more characters, and the character's responses got richer and more varied throughout the study, he questioned if some characters were controlled by a human. In his opinion, the characters' responses should be deterministic and consistent if they were truly autonomous. P114 mentioned that he thought figuring out which characters were controlled by a human could be one of the study objectives. P114 was also the only heavy consumer (more than once a week) of streaming videos hosted by virtual YouTubers. He had relatively richer experience with virtual avatars shown on screen compared with the rest of our participants.

% After being asked about the characters' control, several participants started to question it and gave us several reasons for why they think some characters might be controlled by a human. P121 thought that the human character might be controlled by a human because of the richer facial expressions and more natural movements compared to the others. P103 stated that the robot and the human characters appeared more likely to be human-controlled, due to their high anthropomorphism levels.

% There were also 3 participants who insisted that they didn't think any of the characters could be teleoperated. All of them expressed their high expectation for teleoperated virtual characters compared to a fully autonomous one. \textit{"(P101) Sometimes they could respond, and sometimes they couldn't. If there was a human back there, they should respond to all of the things."}\textit{"(P109) I think (if the characters are controlled by a human) they would've done a better job. Like immediately switching the expression, that I was portraying."}. This shows a higher expectation was posed by the participants for the teleoperated interactive agents compared with the autonomous ones.



% Our study also showed that subjects may unconsciously mirror the character's gestures, effectively leading to a bidirectional imitation loop. Leveraging this loop and controlling it could have interesting applications for emotional therapy or general bonding between the character and the user.






 



==> Sections/futurework.tex <==

\subsection{Use Cases}
As digital characters transition from video games and labs to mainstream displays, the need for fluent communication with non-expert users will increase. Virtual characters may take the role of a shopping clerk, a tour guide in a museum, or a tutor in an educational game. In the wild, these agents will need to handle a range of non-verbal communication signals to capture attention, understand, and deliver a service to a range of user types.

As a first example, non-verbal communication can be especially useful for agents on devices deployed in public spaces in which the agent should remain quiet until a verbal interaction is initiated by the user. In those cases, non-verbal behaviors can be exchanged by the user and the agent in order to negotiate the beginning of the interaction.

Secondly, more non-verbal communication options could allow for reducing the amount of verbal interaction needed with a virtual character. It could become possible to swap between verbal interactions when appropriate (e.g. informational conversations), and non-verbal interactions (e.g. catching a passing wave or playful dance while passing by).

Finally, non-verbal communication may be helpful for accessibility. Verbal communication with a virtual character can be difficult for certain populations (e.g. older adults, or those for which automatic speech recognition performs poorly). Adding more non-verbal communication could lower the barrier for usage.

==> Sections/limitation.tex <==
% \subsubsection{Physically Incapability of the Virtual Character}
% The off-the-shelf software that we used brought several technical limitations to this study which restricted the character's physical capability in the following ways: unable to track overlapped/invisible fingers accurately; lack of lower body movement tracking and mapping; could not capture the body/face orientation once the teleoperator turn their body/face over a certain angel.
% Discouraged by the missing of proper feedback, participants' testing behaviors might be changed. In a future study, virtual characters could have a full range of motion and test if the extra degree of freedom changes participants' interactive behaviors and experience.
% The webcam motion capture software could not track and recognize the finger joints well when some of them were not visible to the camera; 
% Due to the lack of ability in moving the lower body, the teleoperator did not move the character from its spot in the center of the screen; 
% Animaze determines the orientation of the head by constantly extracting and tracking the face. This makes it impossible for the teleoperator to turn her head/body over a certain angle, and actions such as turning around and spinning cannot be performed.

% Those technical limitations put a constraint on the character's physical capabilities that might affect the perceived quality of the non-verbal communication. Three participants suggested we should enable the characters to move in space instead of standing in one spot. Actions involving lower body movements (e.g. running, raising legs) were used to test the characters' physical capability by participants as well, and 2 participants reported they wished the characters could move their legs. Three participants indicated that they wished the character could complete a larger range of motions (e.g. turn around). 


% The study, while motivated by interactions between interactive agents including virtual characters and social robots, was only undertaken with virtual agents. The embodied nature of robots is expected to change some aspects of the stimuli observed, for instance, participants might be less likely to punch an embodied robot than a virtual character. It is an exciting direction in which we can investigate the differences between these two distinct yet related social entities in the future.

% P114 suggested we should let the character recognize speech and speak, despite explicitly being asked about "improving the non-verbal interaction between you and the virtual character" during the interview. P109 talked to 5 characters during the interaction because interaction with speech is natural to her, although the interviewer mentioned several times that the characters were unable to respond to any sound. Isolating each modality and investigating them one at a time can help us understand how each independent interactive element shapes and affects the interaction. However, as humans, we use multimodal frameworks to extract useful information during daily interactions. A future study could explore how adding another modality (e.g. non-linguistic utterance, speech) would affect participants' non-verbal behaviors in free interactions.

% Although culture-specific behaviors were observed in this study (e.g. namaste to greet the character), they were rare and were not closely investigated. Thus, another limitation of this study is the lack of cultural diversity among the participants. 

% Another limitation we have is that in this study only the behaviors elicited by the participants were studied, but not the character's responses. To better understand how participants perceive and evaluate the interaction, in future, we can also take a closer look at the behavioral patterns of the virtual characters.
